Handling Initial Conditions in Vector Fitting for Real Time Modeling of Power System Dynamics

This paper develops a predictive modeling algorithm, denoted as Real-Time Vector Fitting (RTVF), which is capable of approximating the real-time linearized dynamics of multi-input multi-output (MIMO) dynamical systems via rational transfer function matrices. Based on a generalization of the well-known Time-Domain Vector Fitting (TDVF) algorithm, RTVF is suitable for online modeling of dynamical systems which experience both initial-state decay contributions in the measured output signals and concurrently active input signals. These adaptations were specifically contrived to meet the needs currently present in the electrical power systems community, where real-time modeling of low frequency power system dynamics is becoming an increasingly coveted tool by power system operators. After introducing and validating the RTVF scheme on synthetic test cases, this paper presents a series of numerical tests on high-order closed-loop generator systems in the IEEE 39-bus test system.

==> 1-Introduction_Original.tex <==
\IEEEPARstart{D}{ue} to the aggressive deployment of Wide Area Monitoring Systems (WAMS), a deluge of time series data streams are emerging from modernizing smart grids. For instance, as of 2017, Operating Procedure No. 22 specifies that all generation above 100MW in the ISO New England system must provide Phase Measuring Unit (PMU) observability at the point of interconnection~\cite{Vaiman:2018}. Similarly, the 2018 Nodal Operating Guide specifies that all new generators above 20MVA in the ERCOT (Texas) system must provide PMU observability~\cite{ERCOT:2018}. In order to both capitalize on these data streams and enforce effective dynamic security assessment (DSA) in the face of a rapidly modernizing energy landscape, the North American Electric Reliability Corporation (NERC) implemented the so-called MOD-033-1 directive in July of 2017~\cite{NERC_Slides:2016}. Not only does ``MOD33" mandate the continual development of static and dynamic network planning models, but it also requires that the simulated response of these models be compared to actual time series data collected in the network to validate their accuracy~\cite{Akhlaghi:2020}. Associated procedures must also resolve model prediction aberrations. Traditional ``staged" testing of generator models can be costly and inconvenient, because the generator must go offline~\cite{Li:2017}. Thus, performing model tuning and validation online is particularly valuable.

In the electromechanical frequency range, power system dynamics are still dominated by synchronous generators~\cite{Milano:2018}. A wealth of literature exists on the nonlinear physical modeling of these generators and their associated high-order controllers~\cite{Kundur:1994}. MOD33-flavored tuning and validation of these models, though, still faces a variety of practical obstacles; these include the exclusion of unmodeled dynamics, measurement noise, uncertain physical parameter values, unknown controller changes, and, in the limiting case of linearized modeling, residual nonlinearities and drifting equilibrium points. In recent years, a variety of ``grid-scale" methods have been proposed for the purpose of validating these generator + controller models in the presence of strong network perturbations~\cite{NERC_Slides:2016,Foroutan:2019,Huang:2018,Li:2017,Huang:2013,Wu:2018}. Most of these perform some variation of Kalman filter-based parameter tuning via ``play-back" simulation. 

The vast majority of the proposed modeling and validation algorithms are characterized by two salient features. First, they are parameterized by a physical prior; that is, they leverage the structure of a given physical generator model which can assumably be tuned to explain the full set observed dynamics. Second, these algorithms are typically designed to be deployed in the presence of a sufficiently strong network perturbation (e.g. ground fault). Together, these assumptions allow for a variety of helpful assumptions, such as the neglecting of initial state decay and the availability of a high-fidelity prior. Such algorithmic features, although widespread, can be burdensome if the prior model is incomplete, or if real-time model updates are desired\footnote{Real-time updates can be desirable for a variety of reasons, such as in situ controller tuning or operational decision making. This paper will not explore these applications, but assumes they are potentially valuable for operators.} and no recent perturbation events have occurred.

Predictive modeling algorithms which are free from both of these limitations can provide a variety of advantages. If the modeling of generator systems can be performed by a parameterized ``black box" approximation, then the associated algorithm will be freed from the constraints of a potentially erroneous, or completely unknown, prior model. Additionally, if this algorithm can be implemented in the face of ambient, rather than severe, operating conditions, then updates can be performed on the fly, and otherwise unused PMU data can be transformed into actionable information. %Since ambient excitation typically under-excites the nonlinear dynamics of the true physical model, linearized modeling is the most tenable choice for performing dynamical inference in the presence of ambient fluctuations.

There is a large collection of literature devoted to the creation of linear dynamical black box models from time series data in power systems, primarily at the ``wide-area" level, but also at the individual generator level. Excellent reviews on the topic are provided in~\cite{ Pierre:2012, Dosiek:2013 }. One of the most popular ``modal identification" methods, known as Prony analysis, was first applied to power systems in 1990~\cite{ Hauer:1990}. It was further shown in~\cite{ Pierre:1997} that Prony analysis applied to transient data and Wiener-Hopf linear prediction applied to ambient data could both identify very similar system dynamics. Subsequent publications further refined these methods~\cite{Wies:2003,DosiekEst:2013}, but most of them were focused on identification of system modes (i.e. poles), rather than the full transfer functions. More recent work has focused on building model reduced transfer functions from measured terminal data. Using a simple autoregessive with exogenous input (ARX) model, \cite{Chai:2016} develops a process for computing a dynamic equivalent transfer function with simulated or measured data. Voltage magnitude and frequency are chosen as inputs, whiles active and reactive power flows across lines are chosen as outputs. MIMO transfer function approaches are developed in~\cite{ Zhang:2017}\junk{Zhang:2018}, where poles, zeros, and model order are iteratively perturbed based on a least-squares numerical procedure inside a standard MATLAB toolbox.

Most recently, vector fitting approaches have been leveraged to construct power system models from measured field data. In~\cite{ Banuelos-Cabral:2019 }, authors use the numerical Laplace transform to push the problem into the frequency domain. Next, vector fitting and relative dominant-pole measurements (RDPMs) are iteratively leveraged to build estimations of the system modes. Similarly,~\cite{Schumacher:2018} combines time domain vector fitting and the popular ring down analysis to develop a novel modal estimation routine. In a more generic application, \cite{Jakobsen:2017} uses out-of-the-box \TDVF\ to construct a SISO linear model of a turbine governor system from measured PMU; droop gain values are then captured from the derived model.

The black-box identification of dynamic models from time series data goes far beyond power system applications and is regarded as a well established field~\cite{mon-2015-PM,candy2019model}. As noted, one prominent approach is the Time-Domain Vector Fitting (\TDVF) scheme~\cite{jnl-2003-mwcl-TDVF,jnl-2004-aeu-TDVF,mon-2015-PM}. This approach is applicable for estimating rational models of linear systems, starting from the time domain samples of input and output data. Unfortunately, canonical \TDVF\ has the following restrictions:
\begin{itemize}
    \item The system must be at rest when the data acquisition begins. This guarantees that the input and output data are related by a linear transfer function with no contribution from the zero-input (i.e. initial state decay) response.
    \item For a MIMO system with $P$ ports, only separate modeling of each column of the transfer matrix is possible. This limitation requires that only one of the $P$ input components is acting on the system during the separate modeling periods for each transfer matrix column.
\end{itemize}
Since online modeling requires the unknown system to be characterized (i) during its dynamic evolution and (ii) in the presence of concurrently acting inputs, the above limitations often make \TDVF\ unsuitable for real-time MIMO applications. 

This paper introduces a generalized extension of \TDVF, known as Real-Time Vector Fitting (\RTVF), in order to address these limitations. The remainder of this paper is organized as follows. In Section~\ref{sec:Background}, we recall the basic \TDVF\ scheme in order to provide a framework on which the proposed approach is built. We then present our key contributions, namely: 
\begin{enumerate}
\item In Section~\ref{sec:NewSetting}, we remove the restrictions of the basic \TDVF\ scheme by proposing a new problem setting.
\item In Section~\ref{sec:free evolution}, we develop a first generalization of the basic \TDVF\ scheme by removing the requirement of pure zero-state conditions, hence allowing for the presence of non-vanishing initial conditions.
\item In Section~\ref{sec:RTVF}, we develop a second generalization by allowing all input components to act concurrently in the time series data sets used to train the \RTVF\ model.
\end{enumerate}
In Section~\ref{sec:Implementation},
we provide implementation details\junk{\color{SG}, including a discussion on computational cost}. Numerical results, based on several examples, are given in Section~\ref{sec:Results}.




==> 7-Results_Extended.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Computational Cost: Verification}\label{sec:cost_results}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


We start by confirming the theoretical analysis of the computational cost of the \RTVF\ scheme in~\eqref{eq:cost}. A numerical simulation campaign was setup by processing a collection of randomly-generated synthetic $P\times P$ systems with increasing number of ports $P$ ranging from $6$ to $60$, and fixing the model order to $N=8$. Random input and output signals were generated with $K=5000$ samples. All numerical simulations were performed using a Workstation equipped with a 3.3~GHz CPU and 32~GB of RAM.

The time required to perform a single \RTVF\ iteration was recorded as a function of $P$. Figure~\ref{fig:Complexity} compares the actual execution time to the theoretical estimate~\eqref{eq:cost}, demonstrating good asymptotic agreement. Note that for small $P$ the relative contribution of all other algorithm steps is more significant, yet the overall processing time is fraction of a second in such cases.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{./Figures/PortsComplexity.eps}
     \caption{Numerical verification of the \RTVF\ computational cost.}
    \label{fig:Complexity}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Consistency} \label{subsec:consistency}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We tested the \RTVF\ consistency by running a systematic experimental campaign over a set of synthetic randomly generated linear time invariant reference systems, with the objective of checking whether \RTVF\ can provide accurate estimates of all system poles. All the modeled systems share the same dynamic order $N=10$, but have different sizes, with $P$ ranging from~2 to~30.

For each system, a set of virtual input-output measurements was obtained according to the following procedure. The sampling frequency of the input $F_s$, was chosen to be $10$ times the angular frequency $\omega_{\rm{max}}$ of the fastest pole of the reference system. For each input channel, a white noise signal was generated and colored by means of a first order filter with cut-off frequency $\omega_{\rm{max}}$. The top panel in Fig.~\ref{fig:inputOutputSignals} depicts one input signal realization. The output data were collected by exciting each nominal reference system with such inputs, and recording the corresponding outputs. The total number of collected samples was fixed to $K=5000$. In order to simulate the effect of non-zero initial conditions, we ran the \RTVF\ algorithm discarding the first $250$ collected samples. 
\junk{{\color{red}\RTVF\ iterations were stopped through condition~\eqref{eq:denCoeffStop}, with $\epsilon = 10^{-9}$.}}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{./Figures/ModelingWindow.eps} 
    
    \vspace{0.5cm}
    
    \includegraphics[width=\columnwidth]{./Figures/DataVSModel.eps}
     \caption{Top panel: a realization of the input signal used for the identification of the synthetic reference systems. Bottom panel: comparison between computed model output and training samples for one of the test cases. In both panels, the first time window is not used for model generation. The perfect match between model and data output samples in this early window confirms the prediction capabilities of the \RTVF\ model.}
    \label{fig:inputOutputSignals}
\end{figure}



Three metrics were considered to assess the performance of the \RTVF\ identification:
\begin{itemize}
    \item the consistency of the poles estimates, here measured by the Haussdorf distance\footnote{%
    The \emph{Haussdorf distance} or \emph{set distance} between two sets $\mathcal{P}$ and $\mathcal{Q}$ is defined as
    \begin{equation}
    d_H(\mathcal{P},\mathcal{Q})=\max \{ \sup_{p \in \mathcal{P}} \, \inf_{q \in \mathcal{Q}} ||p-q|| , \,  \sup_{q \in \mathcal{Q}} \, \inf_{p \in \mathcal{P}} ||p-q|| \},
    \end{equation}
    }\ %
    $d_H(\mathcal{P},\mathcal{Q})$ between the set of exact poles $\mathcal{P}= \{ p_1, \dots, p_{N} \}$ of the true system and the set $\mathcal{Q}= \{ q_1, \dots, q_{N} \}$ of the numerically computed poles;
    %
    \item the worst-case output error, computed as
    \begin{equation}
        E_{\infty}=\max_{i=1,\dots,P} \max_{k=1,\dots, K}  |y_i(t_k)-\data{y}_i(t_k)|,
    \end{equation}
    where $y_i$ and $\data{y}_i$ are the $i$-th components of the output samples returned by the model and the corresponding training samples, respectively;
    %
    \item the RMS-normalized maximum error, computed as
    \begin{equation}
        E^{\rm RMS}_\infty=\max_{i=1,\dots,P} \max_{k=1,\dots, K} \sqrt{K} \left(\frac{ |y_i(t_k)-\data{y}_i(t_k)|}{||\data{\vet{y}}_i||_2} \right).
    \end{equation} 
\end{itemize}

The experiments showed that the \RTVF\ recovered the system poles almost exactly, with a set distance $d_H(\mathcal{P},\mathcal{Q}) \leq 10^{-10}$ for all the $29$ test cases. Similar results were obtained from the output errors: both $E_{\infty}$ and $E^{\rm RMS}_\infty$ resulted less than $10^{-11}$. As the bottom panel of Fig.~\ref{fig:inputOutputSignals} shows, there is no practical difference between model and data output samples. We conclude that in this ideal identification setting, the performance of the \RTVF\ is excellent for all investigated metrics.

To check the consistency of \RTVF\, we also simulated the presence of measurement noise on the input and output signals, in the case $P=2$ and $N=10$. 
The signal corruption was performed as follows. Let $\smallsignal{x}$ be any of the input or output small signal vectors and let $\alpha$ be a desired level of signal to noise ratio ({\rm SNR}). Then a noise-corrupted signal $\smallsignal{x}_N$ was defined as
\begin{equation}
    \smallsignal{x}_N=\smallsignal{x}+\vet{x}_n
\end{equation}
where $\vet{x}_n$ is a vector of zero-mean gaussian random variables such that:
\begin{equation}
\alpha={\rm SNR}=20\log\frac{{\rm RMS}\{\smallsignal{x}\}}{{\rm RMS}\{\vet{x}_n\}}
\end {equation}
For our experiments we considered increasing levels of ${\rm SNR}$, ranging from $10$ to $100$, with a resolution of $2$.

In order to obtain statistically meaningful results of the modeling accuracy metrics, $R=50$ different synthetic systems where modeled for each prescribed level of $\rm{SNR}$ on the input and output signals.

For each of these $r=1,2,...,R$ models, and for each of the two system output, we computed the \emph{Signal to Error Ratio} ({\rm SER}):
\begin{multline}
     {\rm SER}^r_i=20\log{\frac{{\rm RMS}\{\smallsignal{y}^r_i\}}{{\rm RMS}\{\smallsignal{y}^r_i-\tilde{\vet{y}}^r_{M,i}\}}}  \\    r=1,2,...,R. \qquad i=1,2.
\end{multline}
Here $\smallsignal{y}^r_i$ is the vector of the small signal data samples related to the $i$-th output of the $r$-th system, while $\tilde{\vet{y}}^r_{M,i}$ is the vector of the samples of the $i$-th output of the corresponding model.
The overall time domain accuracy indices are obtained by averaging the above outcomes over all of the $50$ models:
\begin{equation}\label{eq:SER}
     {\rm SER}_i=\frac{1}{R}\sum_{r=1}^R {\rm SER}^r_i  \qquad i=1,2.
\end{equation}
As the {\rm SNR} relates the power of the noise with the power of the reference signal, so the {\rm SER} relates the power of the modeling error to the one of the reference. Therefore, high values of {\rm SER} imply high accuracy of the model against the time domain reference.

In Fig.~\ref{fig:SNR_SER_Synthetic} we report the trend of  ${\rm SER}_1$ and  ${\rm SER}_2$ as functions of the {\rm SNR}. The plot has the following interpretation: when the values of the {\rm SER} and of the {\rm SNR} coincide (solid black line), the power of the modeling error equals the power of the measurement noise, implying unitary sensitivity of the algorithm to the presence of the disturbance. The meaning of the {\rm SER} being above or below the black line threshold is that \RTVF\ is either rejecting or amplifying the presence of the noise on the data.

It can be seen how \RTVF\ shows good noise rejection capabilities, being the {\rm SER} greater to the {\rm SNR} everywhere within the considered interval. The \RTVF\ noise rejection property is expected, since the basis functions entering the fitting condition~\eqref{eq:TDVF linearization} are inherently filtered versions of the noisy input and output signals. Thus, the power of the noise which effectively enters the estimation procedure is reduced according to the dynamics of the underlying system.

%This fact implies that the effect of the noise on the estimation procedure is attenuated by the dynamics of the underlying system itself, and that \RTVF\ is less sensitive to output disturbances that can not be reconstructed by filtered versions of the input signals.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{./Figures/SyntheticWithNoise/SER_SNR.eps}
     \caption{The trend of the {\rm SER} against the {\rm SNR} for the two output of the system. As the {\rm SER} is always above the plane bisector (solid black line), the \RTVF\ algorithm is able to reject partially the presence of measurements noise on the training data. }
     \label{fig:SNR_SER_Synthetic}
\end{figure}

in Fig.\ref{fig:Ex_1_NoisyInputOutput} we report one representative example of noisy input signal with ${\rm SNR}=16$, together with the trend of the model output against the reference model data.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{./Figures/SyntheticWithNoise/InputSNR16.eps}
    \includegraphics[width=\columnwidth]{./Figures/SyntheticWithNoise/OutputValidation.eps}
     \caption{Top panel: an example of noisy input with ${\rm SNR}=16$. Bottom panel: the output of a model generated making use of the noisy signals, against the reference noise-free data.}
     \label{fig:Ex_1_NoisyInputOutput}
\end{figure}

The impact of the measurement noise on the model generation has been also considered in the frequency domain. For a {\rm SNR} level $\alpha$, we computed the following error metrics for each of the $R$ estimated models:
\begin{multline}\label{eq:freqErrorDef}
    E^r_{i,j}=\frac{|| \vet{\data{h}}^r_{i,j}- \vet{h}^r_{i,j} ||_2 }{|| \vet{\data{h}}_{i,j}||_2} 
    \\    r=1,2,...,R. \qquad i,j=1,2.
\end{multline}
where $\vet{\data{h}}^r_{i,j}$ and $\vet{h}^r_{i,j}$ are vectors containing the samples of the $(i,j)$-th entry of the $r$-th reference system and model transfer matrices, respectively. The results have been then averaged over the $R$ test cases to obtain the overall error metrics:
\begin{equation}
    E_{i,j}=\frac{1}{R}  \sum_{r=1}^{R}  E^r_{i,j}
\end{equation}
The results are reported in Fig.~\ref{fig:FreqDomainErrors}. The fitting error is within the $5\%$ accuracy up to ${\rm SNR}=30$. For higher noise power levels, the accuracy in the frequency domain is degraded, although the time domain fitting is still acceptably accurate, as shown in Fig.\ref{fig:Ex_1_NoisyInputOutput}.
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{./Figures/SyntheticWithNoise/ErrorFRequency.eps}
     \caption{The trend of the relative error in the frequency domain as a function of the {\rm SNR}. Each solid line is referred to the error committed by the models over a single element of the target transfer function. The Error is within $5 \%$ for all of the responses up to ${\rm SNR}=30$.}
    \label{fig:FreqDomainErrors}
\end{figure}








% \sgt{Add here an additional analysis of synthetic sistems where both input and output are corrupted by noise (realized exactly as the inputs, but independently added to both inputs and outputs and rescaled by a given amplitude $\sigma$, which can be used as a parameter (signal-to-noise ratio) to check the threshold where \RTVF\ breaks.}

% \sgt{Report the time-domain error in addition to the frequency-donain error. Also, a statistical analysis on a large number of noise realizations must be reported. e.g., report the error (time-frequency for each $\alpha$ computed by averaging on $R$ realizations}

\subsection{IEEE 39-Bus System Results}
In order to test the performance of the \RTVF\ algorithm in a simulated power system setting, we collected data from time domain simulations performed on the IEEE 39-Bus New England system. This system includes 10 generators and 19 nonzero ZIP loads; the associated load, network, and generator models and numerical parameters were taken directly from~\cite{hiskens:2013}. Accordingly, each generator was modeled as a $6^{\rm th}$ order synchronous machine with $3^{\rm rd}$ order automatic voltage regulators and power system stabilizers; additionally, each generator is outfitted with a $3^{\rm rd}$ order turbine governor controller (Type I)~\cite{Milano:2013}. Ultimately, each generator system, with its three controllers, had a total of 15 dynamical states. The interaction between the generator, its controllers, and the network is shown in Fig. \ref{fig:GEN_Sys_BB}. All of the time domain simulations were performed in MATLAB using DAE solver ode23t. Each simulation was initialized from steady state and run for 500 seconds, and the solver's relative and absolute error tolerances were set to $10^{-7}$ and $10^{-8}$, respectively.
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{./Figures/GEN_Sys_BB.pdf}
     \caption{Shown is the interaction between the generator, its three controllers, and the network. The PMU collects data at the generator's point of connection. }
    \label{fig:GEN_Sys_BB}
\end{figure}

\subsubsection*{Load Perturbations}
In order to mimic ambient load fluctuations, we applied an Ornstein-Uhlenbeck (OU) process~\cite{Milano:2013_OU} to the active and reactive power demands at each load. The dynamics of these processes are given by
\begin{align}
\tau\dot{u}_{p} & =- u_{p}+\eta_p\\
\tau\dot{u}_{q} & =- u_{q}+\eta_q,
\end{align}
where $\eta_p$, $\eta_q$ are zero-mean Gaussian variables, and the ``load reversal" time constant $\tau$ was set to 50s. We further applied a low-pass filter (LPF), with a cutoff frequency of $\sim\!\!9$Hz, to the OU variables such that $\hat{u}={\rm LPF}\{{u}\}$. This filtering operation was applied because dynamics above this frequency range become inconsistent with the quasi-stationary phasor approximation used in modeling the network's dynamics. Therefore, high frequency load behaviour is effectively neglected. Finally, these filtered OU variables were parameterized with a time variable $t$ using a cubic spline interpolation scheme and applied to the individual ZIP loads via
\begin{align}
P(t,{\rm V}) & =P_{0}(1+\alpha\cdot\hat{u}_{p}(t))\bigl(a_{Z}\overline{{\rm V}}^{2}+a_{I}\overline{{\rm V}}^{1}+a_{P}\overline{{\rm V}}^{0}\bigr)\label{eq: P_noise}\\
Q(t,{\rm V}) & =Q_{0}(1+\alpha\cdot\hat{u}_{q}(t))\bigl(b_{Z}\overline{{\rm V}}^{2}+b_{I}\overline{{\rm V}}^{1}+b_{P}\overline{{\rm V}}^{0}\bigr),\label{eq: Q_noise}
\end{align}
where $\overline{{\rm V}}\equiv{\rm V}/{\rm V}_0$. As a final step, scalar variable $\alpha$ in (\ref{eq: P_noise})-(\ref{eq: Q_noise}) was experimentally tuned to a numerical value of $\alpha=50$; this tuning generated load perturbations whose corresponding network voltage perturbations approximately matched those of real PMU data (in terms of signal strength).


For the modeling purpose, we consider as input for the system the voltage magnitude ${\rm V}(t)$ and the voltage phase $\theta(t)$, and as output the current magnitude ${\rm I}(t)$ and the current phase $\phi(t)$, measured at the machine-network interface. 

The RTVF algorithm is applied to the data to obtain a model of order $9$.

As for validation of the model quality, we can refer in this case to both time and frequency domain references provided by the availability of the exact equations of the machine functioning. The frequency response of the model against the analytical linearization of the machine is provided in Fig.~\ref{fig:Frequency Response}, while Fig.~\ref{fig:Time Response} reports the trend of the model output compared with the reference signals.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{./Figures/H11.eps}
    \vspace{0.5 cm}
    \includegraphics[width=\columnwidth]{./Figures/H12.eps}
    \vspace{0.5 cm}
    \includegraphics[width=\columnwidth]{./Figures/H21.eps}
    \vspace{0.5 cm}
    \includegraphics[width=\columnwidth]{./Figures/H22.eps}
     \caption{The accuracy of the model of the generator in the frequency domain when compared to the reference data obtained analytically starting from the machine equations. The accuracy of the fitting is excellent up to $3~\rm{Hz}$, and is kept at reasonable levels up to  $7~\rm{Hz}$ }
    \label{fig:Frequency Response}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{./Figures/OutCurrent.eps}
    \vspace{0.5 cm}
    \includegraphics[width=\columnwidth]{./Figures/OutPhase.eps}
     \caption{The accuracy of the model of the generator in the time domain when compared to the reference data obtained by direct integration of the machine equations. The first 4 seconds of the simulations where not used for model generation and therefore can be considered as validation samples.}
    \label{fig:Time Response}
\end{figure}

The results shows that the model accuracy is excellent in both the time and the frequency domain, even if the model order is near half of the one of the reference machine.

\subsubsection*{Measurement Noise}
In order to gauge the practical effectiveness of the \RTVF\ scheme, it was tested in the presence of PMU measurement noise. Specifically, we applied noise to the voltage and current signals measured by the PMU at the terminal of the generators (i.e. ${\rm V}(t)$, ${\rm I}(t)$, $\theta(t)$, $\phi(t)$). To apply this noise, we utilized the procedure outlined in Algorithm \ref{al:SNR}. In this algorithm, an SNR is first specified, in terms of magnitude ($\rm V$, $\rm I$) signals\footnote{Because phase angles drift aggressively, faithfully defining their ``signal strength" for noise application is not a straightforward procedure.}, and the proper amount of noise is then added, where $\eta(t)$ represents an AWG noise vector. Next, noise with an appropriate standard deviation is applied to the phase signals ($\theta$, $\phi$), such that the total vector error (TVE) in the complex plane would be a circular cloud. In other words, an ``equivalent" amount of noise is applied to both the magnitude and phase data, relative to the specified SNR value. 
\junk{Finally, the noisy voltage and current data are used to compute noisy active $P_n(t)$ and reactive $Q_n(t)$ power signals.}

\begin{algorithm}
		\caption{Measurement Noise Application}\label{al:SNR}
		\small{\begin{algorithmic}[1]
			\INPUT Voltage magnitude ${\rm V}(t)$ and phase ${\theta}(t)$ signals;
			\VOID $\quad\,$ Current magnitude ${\rm I}(t)$ and phase ${\phi}(t)$ signals;
			\VOID $\quad\,$ Desired signal measurement SNR
			\OUTPUT Noisy voltage magnitude ${\rm V}_n(t)$ and phase $\theta_n(t)$;
			\VOID $\quad\;\;\;$ Noisy active $P_n(t)$ and reactive $Q_n(t)$ power signals
            \START 
            %\STATE $\sigma_{{\rm V}} \leftarrow{\rm RMS}\left\{ {\rm V}(t)-{\rm E}\left\{ {\rm V}(t)\right\} \right\}$
            %\STATE $\sigma_{{\rm I}} \leftarrow{\rm RMS}\left\{ {\rm I}(t)-{\rm E}\left\{ {\rm I}(t)\right\} \right\}$
            \STATE $\sigma_{{\rm V}n} \leftarrow{\rm RMS}\left\{ {\rm V}(t)-{\rm E}\left\{ {\rm V}(t)\right\} \right\}\cdot10^{-{\rm SNR}/20}$
            \STATE $\sigma_{{\rm I}n} \leftarrow{\rm RMS}\left\{ {\rm I}(t)-{\rm E}\left\{ {\rm I}(t)\right\} \right\}\cdot10^{-{\rm SNR}/20}$
            \STATE ${\rm V}_{n}(t) ={\rm V}(t)+\sigma_{{\rm V}n}\cdot\eta(t)$
            \STATE ${\rm I}_{n}(t) ={\rm I}(t)+\sigma_{{\rm I}n}\cdot\eta(t)$
            \STATE $\theta_{n}(t)\leftarrow\theta(t)+\sigma_{{\rm V}n}\cdot\eta(t)/{\rm E}\left\{ {\rm V}(t)\right\}$
            \STATE $\phi_{n}(t) \leftarrow\phi(t)+\sigma_{{\rm I}n}\cdot\eta(t)/{\rm E}\left\{ {\rm I}(t)\right\}$
\junk{            \STATE $P_{n}(t) ={\rm V}_{n}(t){\rm I}_{n}(t)\cos(\theta_{n}(t)-\phi_{n}(t))$
            \STATE $Q_{n}(t) ={\rm V}_{n}(t){\rm I}_{n}(t)\sin(\theta_{n}(t)-\phi_{n}(t))$}
            \RETURN $I_{n}(t)$, $\phi_{n}(t)$ 
		\end{algorithmic}}
\end{algorithm} 

The accuracy of the fitting in the time domain for the case in which Algorithm~\ref{al:SNR} is ran with ${\rm SNR}=30$ is reported in Fig.~\ref{fig:SNRoutputGenerator}, while In fig.~\ref{fig:InputSNR30} we show the noise corruption on the voltage magnitude for such a noise level.
The results show how the precision of the fitting in the time domain is kept at acceptable levels even with this level of data noise corruption.


\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{./Figures/GeneratorWithNoise/OutputValidation1.eps}
    \includegraphics[width=\columnwidth]{./Figures/GeneratorWithNoise/OutputValidation_2.eps}
     \caption{The accuracy of the model of the generator test case when the voltage and current magnitude signal are corrupted by measurement noise which guarantees ${\rm SNR}=30$. Top panel: small signal current magnitude. Bottom panel: small signal current phase.}
    \label{fig:SNRoutputGenerator}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{./Figures/GeneratorWithNoise/InputSNR30.eps}
     \caption{The voltage magnitude signal when the noise corruption holds with ${\rm SNR}=30$}
    \label{fig:InputSNR30}
\end{figure}




